ANLIzing the Adversarial Natural Language Inference Dataset

We perform an in-depth error analysis of Adversarial NLI (ANLI), a recently introduced large-scale human-and-model-in-the-loop natural language inference dataset collected over multiple rounds. We propose a fine-grained annotation scheme of the different aspects of inference that are responsible for the gold classification labels, and use it to hand-code all three of the ANLI development sets. We use these annotations to answer a variety of interesting questions: which inference types are most common, which models have the highest performance on each reasoning type, and which types are the most challenging for state of-the-art models? We hope that our annotations will enable more fine-grained evaluation of models trained on ANLI, provide us with a deeper understanding of where models fail and succeed, and help us determine how to train better models in future.

==> tables/main_length_tags_table.tex <==
 
    
\begin{table*}[t]
    \centering
    \small
    %\begin{adjustbox}{max width=\linewidth}
    \begin{tabular}{crrrrrrr}
    \toprule
    \bf Subset & \multicolumn{2}{c}{\textbf{Contexts}} & \multicolumn{2}{c}{\textbf{Statements}} & \multicolumn{2}{c}{\textbf{Reasons}} & \bf Count \\
     & Word$_{Len.}$  & Sent.$_{Len.}$ & Word$_{Len.}$  & Sent.$_{Len.}$ & Word$_{Len.}$  & Sent.$_{Len.}$ & \\
    \midrule
    Numerical       & 5.00 (0.44) & 55.8 (\textbf{10.9}) & 4.66 (\textbf{0.66}) & 11.2 (5.46) &  4.46 (0.68) &  21.6 (12.6) & 467 \\
    Basic           & 4.99 (0.52) & 56.7 (15.2) & 4.78 (0.75) & 10.9 (5.17) &  \textbf{4.62} (0.65) & 21.6 (13.6) & 501\\
    Ref. \& Names   & 4.97 (0.48) & 56.2 (15.4) & 4.66 (0.75) & 9.5 (4.87) &  4.54 (0.68) &  20.5 (13.8) & 288 \\
    Tricky          & 4.96 (\textbf{0.88}) & 55.8 (14.1) & 4.74 (0.78) & 10.8 (5.80) &  4.51 (0.68) &  21.0 (12.8) & 404\\
    Reasoning       & 4.97 (0.48) & 54.8 (13.3) & 4.81 (0.78) & 9.7 (4.40) &  4.53 (0.65) &  \bf 21.9 (14.1) & 1018\\
    Imperfections   & \textbf{4.91} (0.52) & 54.3 (14.3) & 4.73 (\textbf{0.84}) & 9.7 (4.70) &  4.46 (0.67) &  \textbf{19.0 (12.0)} & 201\\ 
    \bottomrule
    \end{tabular}
   %\end{adjustbox}
    \caption{Average length of words and sentences in ANLI on contexts and statements. Average length and standard deviation (in parentheses) are provided for each top-level annotation tag. }
    \label{tab:words}
\end{table*}

==> tables/main_pred_overlap_table.tex <==

\begin{table}[t]
\centering
\small
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lcrrrrrrr}
\toprule
Subset &   Overlaps &  All &  C &      N &      E &     A1 &    A2 &     A3 \\
\midrule
\multirow{4}{*}{Full Dev. Set} & R1$^*$, R2, R3 &   29.45& 27.22 &  28.92 &  32.17 &  18.19 &  29.40 &  45.78 \\
& R1$^*$, R2 & 42.20 &  37.90 &  42.34 &  46.26 &  25.28 &  50.00 &  58.84 \\
& R1$^*$, R3  & 36.61 &  34.52 &  35.97 &  39.30 &  21.39 &  40.20 &  55.02 \\
& R2, R3   & 76.25 &  76.87 &  76.59 &  75.30 &  87.08 &  62.40 &  74.50 \\ \midrule
\multirow{4}{*}{Numerical} & R1$^*$, R2, R3 & & 17.65 &  17.91 &  18.99 &  15.83 &  17.61 &  32.65 \\
& R1$^*$, R2  & &  28.51 &  34.33 &  33.52 &  20.85 &  41.51 &  53.06 \\
& R1$^*$, R3 &  &  25.79 &  23.88 &  25.70 &  18.15 &  31.45 &  44.90 \\
& R2, R3    &  &  75.11 &  74.63 &  74.30 &  89.19 &  53.46 &  67.35 \\ \midrule
\multirow{4}{*}{Reasoning} & R1$^*$, R2, R3 &  & 31.22 &  27.90 &  36.12 &  17.37 &  30.54 &  47.95 \\
& R1$^*$, R2 &  &  41.63 &  42.13 &  48.67 &  25.06 &  52.01 &  59.62 \\
& R1$^*$, R3 &  &  37.10 &  35.39 &  43.73 &  20.60 &  42.28 &  55.84 \\
& R2, R3    &  &  80.54 &  75.84 &  76.43 &  86.85 &  63.09 &  77.60 \\\midrule
\multirow{4}{*}{Basic} & R1$^*$, R2, R3 & & 31.51 &  35.83 &  36.60 &  22.99 &  33.02 &  45.25 \\
& R1$^*$, R2 &  &  45.89 &  49.17 &  53.19 &  31.61 &  58.49 &  60.63 \\
& R1$^*$, R3  & &  36.30 &  40.83 &  45.11 &  27.59 &  38.68 &  53.85 \\
& R2, R3   &   &  77.40 &  78.33 &  72.77 &  86.21 &  62.26 &  73.30 \\\midrule
\multirow{4}{*}{Tricky} & R1$^*$, R2, R3 & & 29.63 &  36.36 &  31.88 &  22.75 &  31.73 &  42.86 \\
& R1$^*$, R2  & &  42.33 &  49.35 &  46.38 &  28.74 &  54.81 &  57.89 \\
& R1$^*$, R3 &  &  36.51 &  41.56 &  39.86 &  28.14 &  38.46 &  51.88 \\
& R2, R3    &  &  74.07 &  77.92 &  71.74 &  85.63 &  59.62 &  70.68 \\\midrule
\multirow{4}{*}{Ref. \& Names } & R1$^*$, R2, R3 & & 31.52 &  30.34 &  32.71 &  20.83 &  28.00 &  46.74 \\
& R1$^*$, R2  & &  51.09 &  47.19 &  47.66 &  34.38 &  53.00 &  58.70 \\
& R1$^*$, R3  & &  40.22 &  41.57 &  42.06 &  23.96 &  43.00 &  57.61 \\
& R2, R3   &   &  70.65 &  65.17 &  70.09 &  81.25 &  53.00 &  72.83 \\\midrule
\multirow{4}{*}{Imperfections} & R1$^*$, R2, R3 & & 31.58 &  34.18 &  40.00 &  27.63 &  24.44 &  48.75 \\
& R1$^*$, R2 &  &  36.84 &  43.04 &  56.92 &  36.84 &  40.00 &  57.50 \\
& R1$^*$, R3 &  &  40.35 &  41.77 &  46.15 &  31.58 &  31.11 &  60.00 \\
& R2, R3  &    &  80.70 &  75.95 &  76.92 &  82.89 &  71.11 &  76.25 \\
\bottomrule
\end{tabular}    
\end{adjustbox}
    \caption{Percent Overlap in Model Predictions. We consider the three models used for ANLI collection \citep{nie2019}. `R\textit{n}' refers to the models used to collect the n$^th$ round, `A\textit{n}' refers to the development set from the n$^th$ round, $^*$ marks a BERT model (as opposed to a RoBERTa ensemble), `C', `N', `E' refer to the gold label subset. Lower numbers suggest more disagreement between models. }
    \label{tab:analysis}
\end{table}
